Fine-Grained Guidance for Retrievers: Leveraging LLMs' Feedback in Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) has proven to be an effective method for mitigating hallucination issues inherent in large language models (LLMs). Previous approaches typically train retrievers based on semantic similarity, lacking optimization for RAG. More recent works have proposed aligning retrievers with the preference signals of LLMs. However, these preference signals are often difficult for dense retrievers, which typically have weaker language capabilities, to understand and learn effectively. Drawing inspiration from pedagogical theories like Guided Discovery Learning, we propose a novel framework, FiGRet (Fine-grained Guidance for Retrievers), which leverages the language capabilities of LLMs to construct examples from a more granular, information-centric perspective to guide the learning of retrievers. Specifically, our method utilizes LLMs to construct easy-to-understand examples from samples where the retriever performs poorly, focusing on three learning objectives highly relevant to the RAG scenario: relevance, comprehensiveness, and purity. These examples serve as scaffolding to ultimately align the retriever with the LLM's preferences. Furthermore, we employ a dual curriculum learning strategy and leverage the reciprocal feedback between LLM and retriever to further enhance the performance of the RAG system. A series of experiments demonstrate that our proposed framework enhances the performance of RAG systems equipped with different retrievers and is applicable to various LLMs.

==> Table/5_ablation.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \multicolumn{1}{l}{\textbf{MMLU}} & \multicolumn{1}{l}{\textbf{PQA}} & \multicolumn{1}{l}{\textbf{FEV.}} & \multicolumn{1}{l}{\textbf{Avg.}} \\ 
\midrule
Contriever & 62.5 & 41.7 & 84.5 & 62.9 \\ 
\midrule
w.o. Relevance & \textbf{63.5} & 43.8 & 85.7 & 64.3 \\
w.o. Comp. & 63.2 & 43.0 & 85.7 & 64.0 \\
w.o. Info. Dens. & 63.1 & 44.0 & 85.2 & 64.1 \\ 
\midrule
Ours & 63.4 & \textbf{44.3} & \textbf{85.8} & \textbf{64.5} \\ 
\bottomrule
\end{tabular}
\caption{
Performance of FiGRet when removing each of the three aspects, respectively.
}
\label{tab: ablation}
\end{table}

==> Table/5_main_results.tex <==
\begin{table*}[ht]
\centering
\small
% \resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\midrule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{MMLU}} & \multirow{2}{*}{\textbf{NQ}} & \multirow{2}{*}{\textbf{PQA}} & \multirow{2}{*}{\textbf{HoPo}} & \multirow{2}{*}{\textbf{FEV.}} & \multirow{2}{*}{\textbf{All Avg.}} \\ \cline{2-6}
 & Hum. & Soc. & STEM & Other & All &  &  &  &  &  \\ 
\midrule
\multicolumn{11}{l}{\textit{GPT-3.5-Turbo}} \\ 
\midrule
No retrieval & 52.9 & 76.6 & 53.1 & 75.7 & 63.4 & 48.1 & 44.3 & 33.6 & 82.1 & 54.3 \\
Contriever & 55.1 & 76.3 & {\ul 54.5} & 74.5 & 64.2 & 48.8 & 45.6 & 39.0 & 89.4 & 57.4 \\
AAR$_{\text{Contriever}}$ & 54.3 & {\ul 78.5} & 52.5 & {\ul 77.1} & 64.4 & 49.0 & 46.3 & 36.9 & 89.6 & 57.2 \\
BGE & 52.9 & 78.2 & 54.0 & 76.5 & 64.1 & {\ul 50.3} & 43.9 & 39.5 & 89.3 & 57.4 \\
SBERT & 54.1 & 77.9 & 52.8 & \textbf{77.4} & 64.5 & 49.4 & \textbf{50.1} & 38.7 & 88.5 & 58.2 \\ 
\midrule
FiGRet$_{\text{Contriever}}$ (Ours) & {\ul 55.4} & 76.9 & {\ul 54.5} & {\ul 77.1} & 65.0 & 49.6 & {\ul 48.0} & {\ul 39.9} & \textbf{90.6} & \textbf{58.6} \\
FiGRet$_{\text{BGE}}$ (Ours) & \textbf{55.8} & \textbf{79.8} & 54.3 & 76.5 & \textbf{65.5} & \textbf{50.4} & 45.7 & \textbf{40.0} & {\ul 90.3} & {\ul 58.4} \\
FiGRet$_{\text{SBERT}}$ (Ours) & \textbf{55.8} & 77.2 & \textbf{55.2} & 76.8 & {\ul 65.4} & 49.9 & \textbf{50.1} & 39.1 & 88.7 & \textbf{58.6} \\ 
\midrule
\multicolumn{11}{l}{\textit{Llama-3-8B-Instruct}} \\
\midrule
No retrieval & 52.9 & 74.4 & 51.6 & 73.3 & 62.0 & 33.1 & 26.1 & 25.9 & 79.1 & 45.2 \\
Contriever & 52.9 & 76.3 & 52.5 & 73.3 & 62.5 & 41.3 & 41.7 & 36.0 & 84.5 & 53.2 \\
AAR$_{\text{Contriever}}$ & 52.9 & {\ul 77.2} & {\ul 54.0} & 73.9 & 63.2 & 42.1 & 42.3 & 35.3 & 85.2 & 53.6 \\
BGE & {\ul 54.4} & 76.9 & 52.8 & 73.6 & 63.3 & {\ul 44.1} & 36.1 & 35.9 & 86.1 & 53.1 \\
SBERT & 53.9 & 76.6 & \textbf{54.6} & 73.3 & 63.4 & 41.7 & {\ul 46.0} & 35.7 & {\ul 86.2} & 54.6 \\ 
\midrule
FiGRet$_{\text{Contriever}}$ (Ours) & 53.5 & \textbf{77.5} & 53.1 & {\ul 74.8} & 63.4 & 42.6 & 44.3 & \textbf{36.9} & 85.8 & 54.6 \\
FiGRet$_{\text{BGE}}$ (Ours) & 53.9 & 76.3 & 53.4 & \textbf{75.1} & {\ul 63.6} & \textbf{44.3} & 41.4 & \textbf{36.9} & \textbf{87.4} & {\ul 54.7} \\
FiGRet$_{\text{SBERT}}$ (Ours) & \textbf{54.6} & 76.3 & {\ul 54.0} & 74.2 & \textbf{63.7} & 42.8 & \textbf{46.3} & {\ul 36.1} & {\ul 86.2} & \textbf{55.0} \\ 
\midrule
\multicolumn{11}{l}{\textit{Claude-3-Haiku}} \\ 
\midrule
No retrieval & 59.5 & 82.6 & 59.4 & 78.3 & 68.8 & 27.6 & 31.7 & 26.9 & 70.4 & 45.1 \\
Contriever & 61.6 & 82.0 & {\ul 60.0} & {\ul 79.8} & 70.0 & 35.7 & 41.3 & 33.0 & 90.0 & 54.0 \\
AAR$_{\text{Contriever}}$ & 62.6 & {\ul 83.5} & 59.1 & 79.5 & {\ul 70.2} & 36.1 & 42.1 & 32.7 & {\ul 90.2} & 54.3 \\
BGE & 61.4 & 82.0 & 58.5 & 77.4 & 69.0 & {\ul 38.1} & 37.5 & 33.0 & 89.6 & 53.4 \\
SBERT & 62.0 & 81.0 & 58.8 & 79.2 & 69.4 & 35.9 & {\ul 46.2} & 32.7 & 89.5 & 54.7 \\ 
\midrule
FiGRet$_{\text{Contriever}}$ (Ours) & 62.9 & 82.0 & \textbf{60.3} & \textbf{80.1} & \textbf{70.5} & 36.5 & 44.2 & {\ul 33.3} & \textbf{90.4} & 55.0 \\
FiGRet$_{\text{BGE}}$ (Ours) & {\ul 63.3} & 82.9 & 57.9 & 78.9 & 69.9 & \textbf{40.0} & 42.2 & \textbf{34.7} & 90.0 & {\ul 55.4} \\
FiGRet$_{\text{SBERT}}$ (Ours) & \textbf{63.7} & \textbf{84.2} & 59.4 & 77.7 & \textbf{70.5} & 37.1 & \textbf{46.6} & 33.0 & 90.1 & \textbf{55.5} \\ 
\midrule
\bottomrule
\end{tabular}
% }
\caption{
Our main results on different tasks. We conducted experiments on three different LLMs. Results are reported for our framework initialized with three different base retrievers. For datasets other than MMLU, we tested using 1,000 samples and employed stratified equidistant sampling to ensure fairness. \textbf{Bold} scores represent the best performance within the same LLM, while {\ul underlined} scores represent the second best.
}
\label{tab: main}
\vspace{-10pt}
\end{table*}
